Competing Mechanisms at Vibrated Interfaces of Density-Contrast Fluids

Fluid--fluid interfacial instability and subsequent fluid mixing are ubiquitous in nature and engineering. The hydrodynamic instability of fluid interfaces has long centered on the pressure gradient-driven long-wavelength Rayleigh--Taylor instability and the resonance-induced short-wavelength Faraday instability. However, neither instability alone can explain the dynamics when both mechanisms are present. We identify a previously unseen multi-modal instability emerging from their coexistence. When the denser fluid is polydimethylsiloxane, the mixed region at a high density contrast (Atwood number=0.9) spans a vibration amplitude range approximately twice the gravitational acceleration. Using Floquet stability analysis, we show how vibrations govern transitions between the RT and Faraday instabilities, leading to contention between these instabilities rather than resonant enhancement. The initial transient growth is represented by the exponential modal growth of the most unstable Floquet exponent, along with its accompanying periodic behavior. Direct numerical simulations validate these findings and track interface breakup into the multiscale and nonlinear regimes. Specifically, we show that growing RT modes nonlinearly suppress Faraday responses even when the initial growth rate of the Faraday instability is 3.63 times that of RT, so a bidirectional competition hinders their sustained coexistence.

==> colors.tex <==
\definecolor{lightblue}{rgb}{0.63, 0.74, 0.78}
\definecolor{seagreen}{rgb}{0.18, 0.42, 0.41}
\definecolor{orange}{rgb}{0.85, 0.55, 0.13}
\definecolor{silver}{rgb}{0.69, 0.67, 0.66}
\definecolor{rust}{rgb}{0.72, 0.26, 0.06}
\definecolor{purp}{RGB}{68, 14, 156}

\colorlet{lightrust}{rust!50!white}
\colorlet{lightorange}{orange!25!white}
\colorlet{lightlightblue}{lightblue}
\colorlet{lightsilver}{silver!30!white}
\colorlet{darkorange}{orange!75!black}
\colorlet{darksilver}{silver!65!black}
\colorlet{darklightblue}{lightblue!65!black}
\colorlet{darkrust}{rust!85!black}
\colorlet{darkseagreen}{seagreen!85!black}

==> math_symbols.tex <==
\usepackage{bm}

\usepackage{xparse}
\DeclareDocumentCommand{\diff}{O{} m}{
	\frac{\mathrm{d} #1}{\mathrm{d}#2}
}
\DeclareDocumentCommand{\difftwo}{O{} m}{
	\frac{\mathrm{d}^2 #1}{\mathrm{d}#2^2}
}
\DeclareDocumentCommand{\pdiff}{O{} m}{
	\frac{\partial #1}{\partial #2}
}
\DeclareDocumentCommand{\pdifftwo}{O{} m}{
	\frac{\partial^{2} #1}{\partial #2^{2}}
}
\DeclareDocumentCommand{\integral}{O{} O{} m O{x}}{
	\int_{#1}^{#2} #3\ \mathrm{d}#4
}

\DeclareDocumentCommand{\bu}{}{\bm{u}}
\DeclareDocumentCommand{\bI}{}{\bm{I}}
\DeclareDocumentCommand{\bg}{}{\bm{g}}
\DeclareDocumentCommand{\bq}{}{\bm{q}}
\DeclareDocumentCommand{\bF}{}{\bm{F}}
\DeclareDocumentCommand{\bzeta}{}{\bm{\zeta}}

\DeclareMathOperator*{\argmin}{arg\,min} % thin space, limits underneath in displays

\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\At}{\mathrm{At}}

\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmi}{\mathrm{i}}
\DeclareMathOperator*{\argmax}{arg\!\max}
\newcommand{\transpose}{\mathsf{T}}

==> preamble.tex <==
\makeatletter
  \long\def\pprintMaketitle{\clearpage
  \iflongmktitle\if@twocolumn\let\columnwidth=\textwidth\fi\fi
  \resetTitleCounters
  \def\baselinestretch{1}%
  \printFirstPageNotes
  \begin{center}%
 \thispagestyle{pprintTitle}%
   \def\baselinestretch{1}%
    {\large\bf\@title}\par\vskip5pt
    \normalsize\elsauthors\par\vskip5pt
    \footnotesize\itshape\elsaddress\par\vskip10pt
    % \hrule\vskip12pt
    % \ifvoid\absbox\else\unvbox\absbox\par\vskip10pt\fi
    % \ifvoid\keybox\else\unvbox\keybox\par\vskip10pt\fi
    % \hrule\vskip12pt
    \end{center}%
  \gdef\thefootnote{\arabic{footnote}}%
  }
\makeatother

% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }
% \raggedbottom

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{epsf}
\usepackage{setspace}
\usepackage{soul}
\usepackage[margin=1in]{geometry}
\usepackage{booktabs}
\usepackage[version=4]{mhchem}
\usepackage{array} 
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{xcolor}
\usepackage{wrapfig}
\usepackage{physics}
\usepackage{multirow}
% \usepackage{longtable}

\usepackage{tikz}

\usepackage{tabularx}
% \setlength\LTleft{0pt} 


\usepackage[]{siunitx}
\sisetup{
    separate-uncertainty = true,
    print-unity-mantissa=false,
    per-mode=symbol,
    range-phrase = \text{--}
}

\usepackage{setspace}
\setstretch{1.1}

\usepackage[]{microtype}

\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}

\input{colors.tex}

\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
}

\usepackage[nameinlink]{cleveref}
\crefname{equation}{}{}
\usepackage{empheq}

\usepackage[parfill]{parskip}

\input{math_symbols.tex}

\newcommand{\baw}[1]{\textcolor{rust}{[[Ben says: #1]]}}
\newcommand{\shb}[1]{\textcolor{seagreen}{[[Spencer says: #1]]}}
\newcommand{\spencer}[1]{\textcolor{seagreen}{[[Spencer says: #1]]}}
\newcommand{\todo}[1]{\textcolor{red}{[[To-do: #1]]}}




% \usepackage{titlesec}

% \titleformat{\section}[runin]
%   {\bfseries}{\thesection}{0em}{}[]
